Radio luminosity function of brightest cluster galaxies

By cross-matching the currently largest optical catalog of galaxy clusters and the NVSS radio survey database, we obtain the largest complete sample of brightest cluster galaxies (BCGs) in the redshift range of 0.05<z<0.45, which have radio emission and redshift information. We confirm that more powerful radio BCGs tend to be these optically very bight galaxies located in more relaxed clusters. We derived the radio luminosity functions of BCGs from the largest complete sample of BCGs, and find that the functions depend on the optical luminosity of BCGs and the dynamical state of galaxy clusters. However, the radio luminosity function does not show significant evolution with redshift.

==> tab6.tex <==
\begin{table}
\setlength{\tabcolsep}{1.5mm}
{\footnotesize
\begin{center}
\caption{Fitting parameters of radio luminosity functions of BCG samples.}
\begin{tabular}{lcrrl}
\hline
\hline
\mc{1}{l}{BCG Sample} &\mc{1}{c}{$C_{0}$} &\mc{1}{c}{$P_{0}$} &\mc{1}{c}{$\alpha$} &\mc{1}{c}{$\beta$}\\
%\mc{1}{l}{ } &\mc{1}{c}{$10^{-9}\rm~Mpc^{-3}~dex^{-1}$} &\mc{1}{c}{$10^{24}\rm~W~Hz^{-1}$} &\mc{1}{c}{ } &\mc{1}{c}{ }\\
\hline
All                            & 8.9$\pm$1.2  &38.4$\pm$4.8 &3.18$\pm$0.61 &0.07$\pm$0.05       \\
$M\rm_{r}^{e}\ge-23.3$          &10.2$\pm$1.1  &30.8$\pm$2.7 &4.18$\pm$0.79 &0.11$\pm$0.04       \\
$M\rm_{r}^{e}<-23.3$            &10.9$\pm$2.1  &40.6$\pm$8.5 &2.69$\pm$0.66 &0.00$\pm$0.08       \\
$35<R\rm_{L*}\le45$             &10.9$\pm$1.1  &31.4$\pm$3.1 &3.08$\pm$0.41 &0.06$\pm$0.04       \\
$R\rm_{L*}>45$                  & 9.8$\pm$1.4  &39.7$\pm$5.6 &3.09$\pm$0.60 &0.07$\pm$0.06       \\
$M_{\rm r,2}-M_{\rm r,1}\le0.7$    &10.4$\pm$1.2  &31.0$\pm$2.9 &3.81$\pm$0.63 &0.09$\pm$0.05       \\
$M_{\rm r,2}-M_{\rm r,1}>0.7$      &10.0$\pm$1.4  &45.7$\pm$6.5 &3.04$\pm$0.60 &0.03$\pm$0.06       \\
\hline
\mc{5}{l}{Notes: $C_{0}$ in $10^{-9}\rm~Mpc^{-3}~dex^{-1}$, $P_{0}$ in $10^{24}\rm~W~Hz^{-1}$.}
\end{tabular}
\end{center}
\label{tab5}
}
\end{table}

